Do Knowledge and Reasoning Oriented Benchmarks Induce Stable Representation Signatures in LLMs?

Internal signatures could support monitoring, adaptive computation, and mechanistic analysis, but benchmark prompts can be separable without any shared computational distinction. We test whether a prespecified knowledge/reasoning label defines a reusable internal signature in five contemporary 7B to 31B models. We treat the \textbf{task} as the unit of inference probes hold out complete tasks, labels are permuted across tasks, and the best layer and stream are reselected for every permutation. Raw probes recover an eight-versus-eight-subject MMLU partition in all five models (macro-F1 $0.78$--$0.81$), but prompt text predicts it nearly as well: under an identical probe configuration, the activation advantage is only $0.017$--$0.070$ macro-F1 and is not significant. At the prespecified $0.01$ level, lexical adjustment removes significance while the adjusted states still identify individual subjects, and the selected site changes across task panels and selection rules. Additionally, two released base-training trajectories show no common direction. These pooled layerwise measures recover the task label but identify no transferable knowledge/reasoning signature at the tested sensitivity, which cannot exclude moderate effects. The resulting protocol gives future internal monitors and intervention studies a sequence of tests to pass. Project page: \url{https://parsa-ra.github.io/lmbehave/}.

==> camera_ready.tex <==
% Named build that keeps the NeurIPS checklist appended. The workshop camera-ready itself is
% main.tex (no checklist); use this file only if the organizers request the checklist.
\def\cameraready{1}
\input{capability_knowledge_statistics.tex}


==> main.tex <==
% Overleaf entry point and final camera-ready build: named authors, workshop footer, project
% page link, and no NeurIPS checklist. The substantive source stays in the descriptive filename
% so links from the research repository remain stable.
\def\cameraready{1}
\def\arxivversion{1}
\input{capability_knowledge_statistics.tex}


==> review.tex <==
% Anonymous review build (line numbers, placeholder authors, checklist). Reproduces the layout
% of the submitted version; never used for the camera-ready.
\input{capability_knowledge_statistics.tex}

